Pipelining the Fast Multipole Method over a Runtime System

Fast Multipole Methods (FMM) are a fundamental operation for the simulation of many physical problems. The high performance design of such methods usually requires to carefully tune the algorithm for both the targeted physics and the hardware. In this paper, we propose a new approach that achieves high performance across architectures. Our method consists of expressing the FMM algorithm as a task flow and employing a state-of-the-art runtime system, StarPU, in order to process the tasks on the different processing units. We carefully design the task flow, the mathematical operators, their Central Processing Unit (CPU) and Graphics Processing Unit (GPU) implementations, as well as scheduling schemes. We compute potentials and forces of 200 million particles in 48.7 seconds on a homogeneous 160 cores SGI Altix UV 100 and of 38 million particles in 13.34 seconds on a heterogeneous 12 cores Intel Nehalem processor enhanced with 3 Nvidia M2090 Fermi GPUs.

==> FMM-background.tex <==
\section{Fast Multipole Method}
\label{sec:fmm}
%Pair-wise particle interactions play an important role in many physical
%problems. Examples are astrophysical simulations, molecular dynamics, the
%boundary element method, radiosity in computer-graphics, dislocation dynamics,
%and many more. All these problems can be modelled mathematically as
%\begin{equation}
%  \label{eq:pairwise_summation}
%  f_i = \sum_{j=1}^N K(x_i, y_j) \, w_j \quad \text{for } i=1,\dots,M. 
%\end{equation}
%Here, pairs of particles, in the following denoted by source and target
%particles, are represented by their spatial position vector
%$x,y\in\mathrm{R}^3$, respectively. Their interaction is determined by means
%of the kernel function $K(x,y)$. The summation in
%Eqn.~(\ref{eq:pairwise_summation}) can also be understood as matrix-vector
%product $\mathsf{f}=\mathsf{Kw}$, where $\mathsf{K}$ is a dense matrix of size
%$M\times N$, hence, the cost grows quadratically.
%
%In the last decades researchers have come up with numerous approaches to
%reduce the cost of this summation. The fast multipole method (FMM) turned out
%to be the most prominent one. The idea is to exploit the kernel functions
%\begin{equation}
%  \label{eq:asymtoticall_smooth}
%  K(x,y) = \mathcal{O}\left(|x-y|^{-n}\right) \quad \text{with } n\in
%  \mathrm{N}^+,
%\end{equation}
%i.e., they belong to the family of asymptotically smooth functions which can be
%approximated efficiently as a truncated series expansion (Taylor, spherical
%harmonics, etc.)
%\begin{equation}
%  \label{eq:degenerate_approx}
%  K(x,y) = \sum_{n=0}^{\ell} g_n(x) h_n(y) + \mathcal{O}(\varepsilon^{-\ell}).
%\end{equation}
%If source and target particles are well separated the error of such
%approximations decays exponentially in $\ell$. Such representations finally
%lead to a data-sparse representation of the dense matrix $\mathsf{K}$.

\subsection{Chebyshev FMM (black-box and generic)}
%Most FMMs are kernel specific (see \dots). We adopt the kernel independent FMM
%presented in \cite{Fong2009}. The authors propose to use a Chebyshev
%interpolation scheme
%\begin{equation}
%  \label{eq:cheb_univariate}
%  f(x) \sim \sum_{m=1}^\ell S_m(x) f(\bar x_m) \quad \text{for } x\in[-1,1]
%\end{equation}
%with
%\begin{equation}
%  \label{eq:interpol_polyn}
%  S_m(x) = \frac{1}{\ell} + \frac{2}{\ell} \sum_{i=1}^{\ell-1} T_i(\bar x_m)
%  T_i(x), 
%\end{equation}
%to approximate the kernel function
%\begin{equation}
%  \label{eq:cheby_interpol}
%  K(x,y) \sim \sum_{m=1}^{\ell} S_m(x) \sum_{n=1}^{\ell} K(\bar x_m, \bar
%  y_n) S_n(y).
%\end{equation}
%Note, in $\mathrm{R}^3$ we use the tensor-product ansatz
%\begin{equation}
%  \label{eq:tensor_interpol}
%  S_m(x) = S_{m_1}(x_1) \otimes S_{m_2}(x_2) \otimes S_{m_3}(x_3).
%\end{equation}
%The cost of computing $S_m(x)$ from Eqn.~\eqref{eq:interpol_polyn} is
%$\mathcal{O}(\ell)$, hence, in $\mathrm{R}^3$ a straightforward implementation
%of Eqn.~\eqref{eq:tensor_interpol} would require $\mathcal{O}(M\ell^4)$
%floating point operations. However, by exploiting the outer-product-like
%representation in \eqref{eq:interpol_polyn} the cost can be reduced to
%$\mathcal{O}(M\ell^3 + \ell^4)$. Moreover, the evaluation of all $\{T_i(\bar
%x)\}$ for $\i=1,\dots,\ell-1$ is the same in all directions. Hence, many
%matrix-vector-products can be reformulated as matrix-matrix-products coupled
%with permutations (use of Blas3).

%\subsubsection{Mathematical kernels (complexity)}

\subsubsection{Efficient M2L operator uses symmetries and multiple SVDs}
%The authors of \cite{Fong2009} propose to compress all possible
%$t=1,\dots,316$ M2L operators $\{\mathsf{K}_t\}$, each of size $\ell^3\times
%\ell^3$, via two big singular value decompositions (SVD). Subsequent algebraic
%transformations lead to an efficient representation as $\mathsf{K}_t \sim
%\mathsf{UC}_t\mathsf{V}^\top$, where $\mathsf{C}_t$ is a matrix of size
%$r\times r$ (the low-rank obtained by the SVD). The matrices $\mathsf{U}$ and
%$\mathsf{V}$ of size $\ell^3 \times r$ are the same for all $t$, hence, their
%application can be shifted to the M2M and L2L operator, respectively. We
%propose a more efficient approach: First, by exploiting symmetries, the $316$
%possible M2L operators can be represented by $16$ only. Second, by applying an
%individual SVD to each of the $16$ remaining M2L operators, we can reduce the
%overall cost. Also this approach allows to compute the at most $316$
%matrix-vector products by not more than $16$ matrix-matrix-products coupled
%with some permutations (use of Blas3).
%
%%\begin{table}[htbp]
%%  \caption{Comparison of obtained low-ranks}
%%  \label{tab:one_or_many_svds}
%%  \centering
%%    \begin{tabular}{c | r | c c}
%%    \toprule
%%    $(\ell,\varepsilon_{\text{SVD}})$ & all $t$ & $(2,0,0)$ & $(3,3,3)$ \\
%%    \midrule
%%    $(5,10^{-5})$ &  67 & 23 &  9 \\
%%    $(7,10^{-7})$ & 150 & 45 & 16 \\
%%    $(9,10^{-9})$ & 269 & 77 & 25 \\
%%    \bottomrule
%%  \end{tabular}
%%\end{table}
%
%In Tab.~\ref{tab:cost_of_one_vs_many_svds} we compare both approaches. The
%first column shows three different accuracies of the method given by $Acc$,
%i.e., $(\ell,\varepsilon_{\text{SVD}}) = (Acc, 10^{-Acc})$ (It turned out in
%several studies to be useful to correlate the interpolation order $\ell$ and
%the truncation error $\varepsilon_{\text{SVD}}$ of the SVD. In other words, by
%solely reducing $\varepsilon_{\text{SVD}}$ or augmenting $\ell$ the method
%does not deliver more accurate results, i.e.~the accuracy is delimited by
%either parameter). The second column in
%Tab.~\ref{tab:cost_of_one_vs_many_svds} shows the obtained low-rank $r_{316}$
%by the first approach and the third column the average low-rank $r_{16}$ of
%our approach. The overall cost of approach (i) is given by $\text{cost}_{316}
%= \mathcal{O}\left(316 \cdot r_{316}^2\right)$ and the cost of approach (ii)
%by $\text{cost}_{16} = \mathcal{O}\left(316 \cdot
%  2\ell^3r_{16}\right)$. Column four shows their ratio, approach (ii) is
%decisively more efficient in terms of
%\begin{enumerate}
%\item floating point operations (better compression)
%\item precomputation and memory (16 small SVDs)
%\item cache reuse (Blas3)
%\end{enumerate}
%\begin{table}[htbp]
%  \caption{Comparison of both optimizations of the M2L operator}
%  \label{tab:cost_of_one_vs_many_svds}
%  \centering
%    \begin{tabular}{c | r r | c}
%      \toprule
%      $Acc$ & $r_{316}$ & $r_{16}$ & cost$_{16}/$ cost$_{316}$\\ 
%      \midrule
%      3 &  19 & 4.750  & 0.71 \\
%      5 &  67 & 11.812 & 0.66 \\
%      7 & 150 & 23.375 & 0.71 \\
%      \bottomrule
%  \end{tabular}
%\end{table}

\subsection{General introduction of FMM and introduction of ScalFMM}

\subsection{...}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "sc12"
%%% End: 


==> hybrid.tex <==
\section{Heterogeneous implementation}
\subsection{GPU kernels (flop rates)}
\subsection{Studies of heterogeneous StarPU FMM}


==> multicore.tex <==
\section{Multicore implementation}
\subsection{CPU kernels (flop rates)}
\subsubsection{Comparison to BlockBlasFMM}
\subsection{FMM on top StarPU}
\subsection{Comparison of OpenMP vs. StarPU FMM}

